Ges3ViG: Incorporating Pointing Gestures into Language-Based 3D Visual Grounding for Embodied Reference Understanding

3-Dimensional Embodied Reference Understanding (3D-ERU) combines a language description and an accompanying pointing gesture to identify the most relevant target object in a 3D scene. Although prior work has explored pure language-based 3D grounding, there has been limited exploration of 3D-ERU, which also incorporates human pointing gestures. To address this gap, we introduce a data augmentation framework-Imputer, and use it to curate a new benchmark dataset-ImputeRefer for 3D-ERU, by incorporating human pointing gestures into existing 3D scene datasets that only contain language instructions. We also propose Ges3ViG, a novel model for 3D-ERU that achieves ~30% improvement in accuracy as compared to other 3D-ERU models and ~9% compared to other purely language-based 3D grounding models. Our code and dataset are available at https://github.com/AtharvMane/Ges3ViG.

==> sec/Alt_Method.tex <==
\section{\aug Framework}
\label{sec:method}

We next describe our augmentation framework --~\aug -- to automatically generate dataset for 3D-ERU. Similar to ScanERU, We aim to use the 3D scenes obtained from ScanRefer dataset and insert a human avatar into it.
\aug consists of two parts: 
    (a)~Pointing gesture augmentation, where we propose a simple automated approach to determine the possible locations to \emph{`impute'} the pointing human avatar, and 
    (b)~Language description generation, where we employ an LLM (Gemini \cite{gemini}) to augment the existing verbal description to account for the pointing gesture. 
These components are descried below. 

\subsection{Pointing Gesture Augmentation with \aug \label{sec:pointing-ges-gen}}

\noindpar{Assumptions made: } We make the following assumptions about the 3D scene: (a)~all scenes in the 3D visual grounding dataset are oriented such that the floor's normal is aligned with the Z axis, (b)~the human avatar mesh is pre-aligned with respect to the `floor' of the scene. If the mesh is not already oriented correctly, software such as CloudCompare \cite{cloudcompare} can be used to adjust it. This orientation process only needs to be performed once per avatar, as the same mesh can be reused across all scenes, and (c)~the floor is level (there are no artifacts like stairs) for a major part of the scene. 

\noindpar{Acquiring realistic human avatars:} Augmenting the scene with a pointing gesture requires generating a human pointcloud that can be augmented into the 3D scene such that the generated human pointcloud performs a pointing gesture towards the target object. We define \emph{pointing gesture} as the imaginary line extending from the avatar's shoulder to the tip of the gesturing hand and further.  
To ensure diversity in the generated human pointclouds, we utilize \hey{xx} models from the SMPL-X dataset \cite{SMPL-X}\hey{can we say how many pointclouds does the smpl-x dataset officially have?}. 
\hey{1 line on what blender is might be helpful.} Using the Blender software along with the SMPL-X Blender extension \cite{Blender}, we generate human models of varying sizes and body shapes, for both males and females. 
Additionally \hey{why additionally....what happened in the previous step then?}, we use samples from the SMPLite-X dataset \cite{SMPLite-X}, to create a total of 12 human models with textures, with an equal split of 6 models per gender. Examples of these models are displayed in Figure \ref{fig:pcds}.

The workflow of the \aug framework is as follows. We first voxelize the scene and determine its boundaries. Then we search for vacant spaces for placing the human avatar such that there is a direct line-of-sight available for pointing at the target. The avatar is then placed in a suitable vacant space and finally a VLM is prompted with the scene images containing the human to generate a language instruction for referring to the target object. These steps are explained in detail below.
%\begin{itemize}[leftmargin=*]
    
\noindpar{Voxelization of the scene:} 
We voxelize the scene to discretize the search space, which allows for efficient querying of point occupancy. Checking occupancy in a voxel grid is much faster compared to meshes or point clouds and voxel grids allow interaction with `empty space'. These empty spaces are crucial, as they define the potential locations where the human avatar can be placed.
We create voxel grid $V_1(\mathbb{N}^3\rightarrow \{0,1 \} )$ which represents the original scene with the target object, and voxel grid $V_2(\mathbb{N}^3\rightarrow \{0,1 \} )$ which represents the scene with the target object removed and  to model un-occupancy. Each voxel $V_i(x,y,z)$ in $V_1$ and $V_2$ is assigned a value of `1' if it is occupied by an object or `0' if it is unoccupied.
We also voxelize the human avatar mesh separately to get a 3D grid (similar dimension as $V_1$ and $V_2$) given by $H(\mathbb{N}^3\rightarrow \{0,1 \} )$. A voxel $H(x,y,z)$ is assigned a value of `1' only if it is occupied by the human. Otherwise it is set to `0'.

\noindpar{Determining scene boundaries: } In this step, we calculate the scene bounds to ensure the human avatar is not placed outside the scene. This is done by identifying the the largest contour in a binary image created by projecting the voxel grid onto the $XY$-plane (as shown in Figure \ref{fig:contour}). Then the voxels (or pixels?) in the binary image that fall inside the boundary are filled with a value 1 and this binary image (Figure \ref{fig:contour_filled}) is stacked up vertically, $h$ times, where $h$ represents the height of the voxel grid. This stacking process creates a 3D binary grid  denoted by a 3D binary function $B(\mathbb{N}^3 \rightarrow {1,0})$.\hey{why is stacking done? Where is this 3D binary grid used in subsequent steps?}

\noindpar{Finding the occupiable regions:} In this step, we identify all regions within the scene that can accommodate a human mesh. To ensure that the feet of the human avatar is placed appropriately \On' the floor of the scene, we need to determine the appropriate co-ordinates of the human feet and the floor level within the voxel grid. We define the ``foot" as the lowest point in the human avatar mesh, denoted as $(x_{foot}, y_{foot}, z_{foot})$ after converting into voxel-scale. Since there are multiple voxels corresponding to `floor', we adopt the following approach to estimate the vertical displacement floor (denoted as ($h_{floor}$) with respect to the origin of the scene. The 3D scenes in ScanRefer dataset are originally from ScanNEtV2. From ScanNetV2 it is possible to obtain a list of vertices that are labelled as `floor'. 
$h_{floor}$ is then calculated by taking the lower of following two values: (1) the average height of all floor vertices plus a offset $C_1 = 0.04$, and (2) the 85\textsuperscript{th} percentile of the height distribution of these points. Next, we convert this estimated height to voxel scale, denoted as $h_{floor\_vox}$. The final floor height estimated is given by $\hat{h}_{floor\_vox} = min(C_2, h_{floor\_vox})$, where $C_2=4$.

We adopt a sliding volume approach to identify sufficiently large vacant spaces that can fit the human avatar. The size of the sliding volume is chosen to be equal to the size of the human avatar voxel grid. We then use the human voxel grid as a mask to check if there is exactly enough space to fit the human avatar at a given a point $(i,j)$ on the floor. 
We consider the human avatar volume $H$ comprising of voxels whose co-ordinates range from  $(i,j,\hat{h}_{floor\_vox})$ to $(i+x_{max}, j+y_{max}, \hat{h}_{floor\_vox}+h_{human\_vox})$. We see that the entire volume falls into a clear space of the scene if it satisfies the condition
    \begin{dmath}\label{eq: occ_points}    \sum_{x=0}^{x_{max}}\sum_{y=0}^{y_{max}}\sum_{z=0}^{z_{max}}H(x,y,z) \shorteq\shorteq \sum_{x=0}^{x_{max}}\sum_{y=0}^{y_{max}}\sum_{z=0}^{z_{max}}{H(x,y,z) \times V_1(i+x,j+y,k+z)}
    \end{dmath}
In practice, we observed that there could some cases of improper human positioning even if after conditions are satisifed (especially after rotation of the avatar) might. Hence, we increase the border widths by $10$ voxels to avoid such scenarios. We store $(i,j,\hat{h}_{floor\_vox}+h_{human\_vox})$ in the set $O_{no\_collide}$ if all the voxels in the volume places at (i,j) on the floor satisfy the condition \ref{eq: occ_points} after accounting for the additional allowance.

%\noindpar{Identifying target co-ordinates: } We define the center of the 3D bounding box of the target object as the origin of the line-of-sight. To ensure an unobstructed view, we temporarily remove the object of interest from the scene, preventing it from acting as an obstacle to the line of sight originating from its center.

\noindpar{Grid visibility search: } In this step we aim to determine whether there exists direct line-of-sight from the center of the target object to the human avatar. We define the center of the 3D bounding box of the target object as the origin of the line-of-sight. To ensure an unobstructed view, we use the voxel grid $V2$ where the target object is removed. This is done so that the center of the target object is not hidden from view by its own boundary surface. Visibility between two points can be determined without directly checking for a line of sight, particularly in grid-based environments \cite{buildingvis}. A path-counting algorithm has been used in 2D to calculate visibility scores for each grid cell, as explored in \cite{gridwalk}. We extend this approach to 3D environments. Given $V_2$, we compute a visibility score grid, denoted as $S(\mathbb{N}^3 \rightarrow \mathbb{R})$, where $S$ is defined as:

\begin{dmath}    
%    S(x,y,z) = V_2(x,y,z) \times\frac{x \times S(x-1,y,z) + y \times S(x,y-1,z) + z \times S(x,y,z-1)}{x+y+z} 
    S(x,y,z) = (\frac{x \times S(x-1,y,z)}{x+y+z} + \frac{y \times S(x,y-1,z)}{x+y+z} + \frac{z \times S(x,y,z-1)}{x+y+z} ) \times V_2(x,y,z)
\end{dmath}

We then obtain $S'(\mathbb{N}^3 \rightarrow \{1,0\})$ a thresholded version of $S$ as follows:
\begin{equation}
        S'(x,y,z)= 
\begin{cases}
    1,&             \text{if } S(x,y,z)\geq0.33\\
    0,              & \text{otherwise}
\end{cases}
\end{equation}
$S'$ gives us a good approximation for all the visible regions. We define the set of all the coordinates where $S'=1$ as the \emph{region of visibility}. Figure \ref{fig:grid_visibility} shows an example of such a region of visibility. A threshold of 0.33 was chosen empirically.

\noindpar{Computing the final transformation matrix: } 
To consider that a 3D pointcloud of the human avatar has been successfully \emph{imputed} in the scene, it must satisfy the following conditions: (a)~\textit{Boundary}--the human avatar is placed within the bounds of the scene, (b)~\textit{Overlap}--the avatar does not occupy any pre-occupied space in the scene, and (c)~\textit{Line-of-sight}--there is a direct unblocked line between the human avatar's gesture and the object of interest in the scene.
For the coordinate $(i,j,k)$ in the voxel grid, the \textit{boundary} condition can be checked by querying the value $B(i,j,k)$. 
If it is $1$, then \textit{boundary} condition is satisfied. 
Similarly, if $(i,j,k) \in O_{no\_collide}$, then, $(i,j,k)$ also satisfies the \textit{overlap} condition. 
If $S'(x,y,z)=1$ then $(i,j,k)$ also satisfies the \textit{ line-of-sight} condition. 
Thus the aim is to new_data_2.append(img)collect all such points. \hey{what is this?} 
These are the potential points where the human point cloud could be augmented. 
We place these points in a container $C_{initial\_samples}.$
We use the gesturing shoulder of the human avatar as a pivot of rotation to point toward the object of interest. It is sufficient to fit the shoulder in the region of visibility since having the pivot inside the region of visibility ensures that after rotation, the entire gesture (in our case, the hand) lies inside the region of visibility.
We construct a set $C_{final\_samples}$ from the points that satisfy the above equation. \hey{when there are multiple vacant spaces that satisfy the three conditions, how does Imputer choose the position of the avatar?}
After finding the coordinates mentioned in the condition above, we calculate simple Euclidean transforms to move the human from its original position to the desired coordinate and then rotate the human in place. 

We have the coordinates of 4 points, each of which we convert to homogeneous coordinates: \begin{enumerate}
    \item The coordinates of the shoulder of the human $\vec{S}=[S_x, S_y, S_z, 1]^T$.
    \item The coordinates of the tip of the pointing gesture $\vec{P}=[P_x, P_y, P_z, 1]^T$.
    \item The coordinates of the desired destination for the human pointcloud $\vec{D}=[D_x, D_y, D_z, 1]^T$ and
    \item The coordinates of the centroid of the bounding box of the 'object of interest' $\vec{B}=[B_x, B_y, B_z, 1]^T$.
\end{enumerate}

We define the translation matrix $\mathbf{M_{t}}$ that moves the human from its current position to the destination as follows:
\begin{equation}
    \mathbf{M_{t}} = \begin{bmatrix}
                                    1 & 0 & 0 & D_x-S_x\\
                                    0 & 1 & 0 & D_y-S_y\\
                                    0 & 0 & 1 & D_z-S_y\\
                                    0 & 0 & 0 & 1
                                    \end{bmatrix}
\end{equation}

We compute $\vec{S'} = \mathbf{M_t}\cdot\ \vec{S}$ and $\vec{P'} = \mathbf{M_t}\cdot\ \vec{P}$ and convert each of the obtained vectors back to cartesian coordinate. We note that $\vec{S'}=\vec{D}$. 

From here, we compute a rotation matrix that, when applied to $\vec{E} = \vec{P'} - \vec{S'}$, aligns the vector with $\vec{F} = \vec{B} - \vec{S'}$. We first get the unit vectors in each direction as $\hat{E}=\frac{\vec{E}}{|\vec{E}|}$ and $\hat{F}=\frac{\vec{F}}{|\vec{F}|}$.
We then define the rotation matrix $\mathbf{M_r}$ as 
\begin{equation}
    \mathbf{M_r}=\mathbf{I} + \mathbf{V} + (\frac{1-\hat{E}^T\cdot \hat{F} \hat{}}{|\vec{V}|^2})( \mathbf{V}^T\cdot\mathbf{V})
\end{equation}
Where $\vec{V} = \hat{E} \times \hat{F} $. Let $\vec{V}=[V_x, V_y, V_z]$
\begin{equation}
    \mathbf{V} = \begin{bmatrix}
                                    0 & -V_z & -V_y \\
                                    V_z & 0 & -V_x \\
                                    V_y & V_x & 0
                    \end{bmatrix}
\end{equation}
Note that $\mathbf{M_r}$ is a $3\times3$ matrix, and that this rotational matrix would rotate the human avatar correctly, if the pivot, i.e. the shoulder, was placed at the origin. To take the shift of the shoulder into account after translation, we use the following final $4\times4$ rotation in homogeneous coordinate:
\begin{equation}
    \mathbf{M_R} = \begin{bmatrix}
    \mathbf{M_r} & \vec{S}-\mathbf{M_r}\vec{S}\\
    0 & 1
    \end{bmatrix}
\end{equation}
This can be easily obtained by the following matrix multiplications.
\begin{equation}
    \mathbf{M_R} = \begin{bmatrix}
    \mathbf{I_{3\times3}} & \vec{S}\\
    0 & 1
    \end{bmatrix}
    \begin{bmatrix}
    \mathbf{M_r} & \vec{0}\\
    0 & 1
    \end{bmatrix}
    \begin{bmatrix}
    \mathbf{I_{3\times3}} & -\vec{S}\\
    0 & 1
    \end{bmatrix}
\end{equation}
Where $\vec{0}$ represents a 3 dimensional vector of length $0$ and $\mathbf{I_{3\times3}}$ represents a $3\times3$ identity matrix.
\par We then store the final matrix $\mathbf{M} = \mathbf{M_R} \cdot \mathbf{M_t}$.

When loading the dataset, we load the scene and the human pointcloud seperately. We then add a rotational jitter of  range $N_{jitter} = 9^{\circ}$ to simulate measurement errors while capturing the human. \hey{reframe this}



Figure \ref{fig:success_impute} shows the human avatar placed in a 3D scene, which is marked by a red box, pointing towards the target object marked by a green box.



\iffalse
% \section{Baseline}
% \label{sec:baseline}
% \begin{itemize}
% \item \dw{I might remove this, since there are already overlapping parts in M3DRefCLIP and \names}
%     \item \textbf{M3DRefClip \cite{m3drefclip}}
%     \par{We use M3DRef-CLIP \cite{m3drefclip} as the baseline model.

%     \par{M3DRef-CLIP is a 2 stage model. It uses an instance segmentation model, PointGroup \cite{pointgroup}, as its detector and feature extractor for the pointclouds. It uses CLIP \cite{clip} to encode the textual data from the CLIP language encoder to get token-level and sentence-level features for the textual data. An online object renderer then renders each output of the object detector into multiview images. These images are fed to the clip image encoder to get the image-based features. Given that there are $M$ renderings of the object, we will have $M\times C$ number of features for each point in the pointcloud for each object. These features are then passed through an MLP to get a single $C$ dimensional feature per point. For each point, these new features are concatenated with the original features obtained from PointGroup. These features, along with the language features, are then passed through a cross-modal transformer-based fusion module to give the final prediction.}
    
    
%     \par{
%     The loss function for M3DRef-CLIP is divided into three parts: the detection loss from the PointGroup \cite{pointgroup} detector, the reference loss, which is a multi-class cross-entropy loss to select objects that the referring expressions refer to, and the symmetric contrastive loss. The detection loss itself is made of 4 different losses: 1) cross-entropy loss for supervising per-point
%     semantic class prediction called the 'semantic loss,' 2) L1 loss for supervising per-point offset vector towards object centers (useful for instance segmentation), called the 'offset norm loss,' 3) A directional loss formed as a mean of minus cosine similarities for further constraining the direction of per-point offset vectors called the 'offset dir loss' and finally 4) A binary cross-entropy loss for supervising per-point objectness confidence score here called the 'score loss.'
%     }
%     }
% \end{itemize}

\section{\aug Framework}
\label{sec:method}

%ScanERU introduced a dataset for gesture-enhanced 3D Visual Grounding, using scenes from ScanNet and incorporating synthetic human avatars pointing at target objects within the scene. 
%To insert the avatars, they conducted a crowd-sourced study, asking participants to select likely locations for the avatars to be placed, ensuring they were oriented toward the target object. 
%The resulting dataset combined the original ScanRefer language descriptions with the modified ScanNet scenes, serving as a benchmark for gesture-enhanced 3D visual grounding. 
% \artharv{We have no evidence to validate claim a), They havent shared the crowdsourced data with us at all, all they've done is capured their own test data where they we very close to the object. The dataset they have given us is realtime captured, not the crowdsourced one.}
% \vig{Pls see the language used in the introduction para 3. We can mention that SCan ERU is no longer publicly accessible, but a portion of the test dataset has been obtained from the authors.}
%However, we identified several key limitations with this approach: 
    %(i)~By relying on participants to choose avatar locations, the dataset is biased. Participants often place the avatar very close to the target object, reducing the task’s difficulty and diminishing the need for detailed language descriptions to identify the target. 
   % (ii)~The crowd-sourced study limits both the nuanced control and scalability of avatar placement. \sou{why not add the language descriptor point here, as that is also a limitation?}
%One must note that we do not have access to the entire dataset (as it is not publicly available), but a part of the test dataset shared with us by the authors.


%To address these limitations, we propose \dataset, generated through an automated \aug framework instead of a manual crowd-sourced approach. 
%This framework not only allows more precise control and scalability in avatar placement, but also increases the difficulty of the task by eliminating the bias of placing the avatar too close to the target object. 

%Additionally, ScanERU used the original ScanRefer language descriptions without modification. 
%However, studies such as \cite{weerakoon2020gesture} have shown that when both verbal descriptions and pointing gestures are used, participants tend to provide less detailed verbal descriptions. 
%To account for this, we propose to augment the existing language descriptions automatically using Gemini, a LLM that understands the presence of pointing gestures. 
%Furthermore, the complete ScanERU dataset is currently unavailable. %, with only a limited number of test samples publicly accessible. 
%This limitation will make our proposed \dataset the only fully publicly available dataset for gesture-enhanced 3D visual grounding, offering broader accessibility for research and development in this domain.
We next describe our augmentation framework --~\aug -- to automatically generate dataset for 3D-ERU. 
\aug consists of two parts: 
    (a)~Pointing gesture augmentation, where we propose a simple yet automated approach to determine the possible locations to \emph{`impute'} the pointing human avatar, and 
    (b)~Language description generation, where we employ an LLM (Gemini \cite{gemini}) to augment the existing verbal description to account for the pointing gesture. 
We next describe both these components. 

\subsection{Pointing Gesture Augmentation with \aug \label{sec:pointing-ges-gen}}
Augmenting the scene with a pointing gesture requires generating a human pointcloud that can be augmented into the 3D scene such that the generated human pointcloud performs a pointing gesture towards the target object. We define \emph{pointing gesture} as the imaginary line extending from the avatar's shoulder to the tip of the gesturing hand and further. 
% We outline our  pointing gesture generation process, where we %\st{impute' a point cloud of a pointing human} 
% compute positions of human pointcloud in the scene. 
%\artharv{since we arent technically using pointclouds in imputer but meshes and voxelgrids}. 
%To collect a diverse set of synthetic 3D human models, 
To ensure diversity in the generated human pointclouds, we utilize \hey{xx} models from the SMPL-X dataset \cite{SMPL-X}\hey{can we say how many pointclouds does the smpl-x dataset officially have?}. 
\hey{1 line on what blender is might be helpful.} Using the Blender software along with the SMPL-X Blender extension \cite{Blender}, we generate human models of varying sizes and body shapes, for both males and females. 
Additionally \hey{why additionally....what happened in the previous step then?}, we use samples from the SMPLite-X dataset \cite{SMPLite-X}, to create a total of 12 human models with textures, with an equal split of 6 models per gender. Examples of these models are displayed in Figure \ref{fig:pcds}.

\noindpar{Conditions for successful augmentation:} To consider that a 3D pointcloud of the human avatar has been successfully \emph{imputed} in the scene, it must satisfy the following conditions: (a)~\textit{Boundary}--the human avatar is placed within the bounds of the scene, (b)~\textit{Overlap}--the avatar does not occupy any pre-occupied space in the scene, and (c)~\textit{Line-of-sight}--there is a direct unblocked line between the human avatar's gesture and the object of interest in the scene.


% We first outline the conditions for successful augmentation of the pointing human avatar:

% \begin{enumerate}[leftmargin=*]\label{sec:success_conds}
%     \item The human avatar is placed within the bounds of the scene.
%     \item The imputed human avatar does not occupy a pre-occupied space in the scene.
%     \item There must be a clear line of sight between the human avatar's gesture and the object of interest in the scene. The pointing line is defined as the imaginary line extending from the avatar's shoulder to the tip of the gesturing hand.
% %    \item The human gesture points to the object of interest. ie., the distance from the pointing line to the center of the target object is $\le XXX$.
% \end{enumerate} 

\noindpar{Assumptions made: } We make the following assumptions about the 3D scene: (a)~all scenes in the 3D visual grounding dataset are oriented such that the floor's normal is aligned with the Z axis, (b)~the human avatar mesh is pre-aligned with respect to the `floor' of the scene. If the mesh is not already oriented correctly, software such as CloudCompare \cite{cloudcompare} can be used to adjust it. This orientation process only needs to be performed once per avatar, as the same mesh can be reused across all scenes, and (c)~the floor is level (there are no artifacts like stairs) for a major part of the scene. 
% We make the following assumptions to enable successful augmentations:
% \begin{enumerate}[leftmargin=*]
%     \item In the 3D visual grounding dataset, all scenes are oriented such that the floor's normal is aligned with the Z axis. 
%     \item The human avatar mesh is pre-aligned with respect to the `floor' of the scene. If the mesh is not already oriented correctly, software such as CloudCompare \cite{cloudcompare} can be used to adjust it. This orientation process only needs to be performed once per avatar, as the same mesh can be reused across all scenes.

%     \item The floor is level (there are no artifacts like stairs) for a major part of the scene.

% \end{enumerate}

The workflow of the \aug framework is as follows. We first determine the center of the target object towards which the pointing gesture will be performed. We then voxelize the scene and determine its boundaries. Then we search for vacant spaces for placing the human avatar such that there is a direct line-of-sight available for pointing at the target. The avatar is then placed in a suitable vacant space and finally a VLM is prompted with the scene images containing the human to generate a language instruction for referring to the target object. These steps are explained in detail below.
\vig {Why do we remove the target object first? and when do we insert it back? IF we remove the target object will it not be counted as vacant space in subsequent steps?}
%\begin{itemize}[leftmargin=*]
\noindpar{Removal of object-of-interest: \hey{suggest to change to `Identifying target co-ordinates'}} We define the center of the 3D bounding box of the target object as the origin of the line-of-sight. To ensure an unobstructed view, we temporarily remove the object of interest from the scene, preventing it from acting as an obstacle to the line of sight originating from its center.
    
\noindpar{Voxelization of the scene:} 
\hey{voxeliation is done after re-inserting the object in the scene?} We voxelize the scene to discretize the search space, which allows for efficient querying of point occupancy. Checking occupancy in a voxel grid is much faster compared to meshes or point clouds and voxel grids allow interaction with `empty space'. These empty spaces are crucial, as they define the potential locations where the human avatar can be placed.

We then define functions $V_1(\mathbb{N}^3\rightarrow \{0,1 \} )$ and $V_2(\mathbb{N}^3\rightarrow \{0,1 \} )$ to model un-occupancy.
where each $V_i$ is defined as follows:
\begin{equation*}
        V_i(x,y,z)= 
\begin{cases}
    1,&             \text{if } (x,y,z) \text{ is unoccupied}\\
    0,              & \text{otherwise}
\end{cases}
\end{equation*}
$V_1$ represents the voxel grid of the original scene, and $V_2$ represents the voxel grid of the scene with the target object removed. 
We also voxelize the human avatar mesh separately to get a 3D grid given by $H(\mathbb{N}^3\rightarrow \{0,1 \} )$ to model the human.
$H$ is defined as follows:
\begin{equation*}
        H(x,y,z)= 
\begin{cases}
    1,&             \text{if } (x,y,z) \text{ is a part of the human}\\
    0,              & \text{otherwise}
\end{cases}
\end{equation*}

\noindpar{Determining scene boundaries: } In this step, we calculate the scene bounds to ensure the human avatar is not placed outside the scene. This is done by identifying the outermost boundaries of the scene, which are determined by the largest contour in a binary image created by projecting the voxel grid onto the $XY$-plane. The process involves projecting the entire scene onto the $XY$-plane and then detecting the largest contour in the resulting image\hey{is this RGB image or a planar voxel grid?}. Figure \ref{fig:contour} illustrates the contour formed by this process. The identified contour is subsequently filled internally with the value 1, after which the image is stacked vertically $h$ times, where $h$ represents the height of the voxel grid. Figure \ref{fig:contour_filled} illustrates the filled contour. This stacking process facilitates the creation of a 3D binary grid. We denote this grid as a 3D binary function $B(\mathbb{N}^3 \rightarrow {1,0})$. \hey{Many possible questions may arise in the reader's mind. What is the use of this binary grid? How did you get a voxel grid by stacking up 2D RGB images?}

\hey{How about this para? -- In this step, we calculate the scene bounds to ensure the human avatar is not placed outside the scene. . This is done by identifying the the largest contour in a binary image created by projecting the voxel grid onto the $XY$-plane (as shown in Figure \ref{fig:contour}). Then the voxels (or pixels?) in the binary image that fall inside the boundary are filled with a value 1 and this binary image (Figure \ref{fig:contour_filled}) is stacked up vertically, $h$ times, where $h$ represents the height of the voxel grid. This stacking process creates a 3D binary grid  denoted by a 3D binary function $B(\mathbb{N}^3 \rightarrow {1,0})$}.


\noindpar{Finding the occupiable regions: } In this step, we identify all regions within the scene that can accommodate a human mesh.
     % \st{we assume a maximum floor height $Z_{floor}=min(C_1, h_{floor})$ voxels, determined empirically. The lowest point of the human avatar must always be above $Z_{floor}$.}}   
     We need to place the human avatar on the floor, ensuring there is no ``collision" \hey{what is collision? feet touching the floor is collision?} between the avatar's feet and the scene's floor. To achieve this, we first estimate the floor height (\hey{do you mean z-coordinate of floor?}) using the following approach. From the set of vertices labeled as "floor" in the ScanNetv2 dataset \cite{dai2017scannet} \hey{why did ScanNetv2 come into picture here? So far we have spoken about ScanRefer only. People wont understand this sentence.}, we calculate the floor height $h_{floor}$. This is done by taking the minimum \hey{why minimum?} of two values: (1) the average height of all floor vertices plus a constant $C_1 = 0.04$ , and (2) the 85\textsuperscript{th} percentile of the height distribution of these points. Next, we convert this estimated height to voxel scale, denoted as $h_{floor\_vox}$. The final floor height estimator is given by $\hat{He}_{floor\_vox} = min(C_2, h_{floor\_vox})$, where $C_2=4$.   \hey{what is He? Is it used later?}. \hey{I think a lot of the deatils can be moved to supplementary material?} 
    % As a first step, we need to place the human avatar on the floor. To avoid any ``collision'' between the floors of the scenes and the foot of the human avatar. We estimate the floor height as follows. From the set of vertices with the floor label provided by the ScanNetv2 \cite{dai2017scannet} dataset, we estimate the floor height $h_{floor}$ as the minimum between the average height of all the vertices added with a constant $C_1 = 0.04$ and the $85th$ percentile in the height of the points. We then convert this height into the voxel scale $h_{floor\_vox}$. The final estimator $\hat{He}_{floor\_vox} = min(C_2, h_{floor\_vox})$ we keep $C_2=4$
    %We define the "foot" as the lowest point in the human avatar mesh, denoted as
    % \par{We then define 'foot' as the lowest point in the human avatar mesh. We call this point $(x_{foot}, y_{foot}, z_{foot})$. We determine the index of the foot $(X_{foot}, Y_{foot}, Z_{foot})$ w.r.t the voxel grid of the scene $V$. This can be done using the following equation}
    We define the "foot" as the lowest point in the human avatar mesh, denoted as $(x_{foot}, y_{foot}, z_{foot})$. To locate this point within the voxel grid of the scene $V$, we determine its corresponding index $(X_{foot}, Y_{foot}, Z_{foot})$ in the voxel grid. This can be calculated using the following equation:
    \begin{equation}
        [X_{foot}, Y_{foot}, Z_{foot}]  = \lfloor x_{foot}/r, y_{foot}/r, z_{foot}/r \rfloor
    \end{equation}
    % \begin{equation*}
    %     Y_{foot} = \lfloor y_{foot}/r \rfloor
    % \end{equation*}
    % \begin{equation*}
    %     Z_{foot} = \lfloor z_{foot}/r \rfloor
    % \end{equation*}
    Here, $r$ is the resolution of voxelization for the scene voxel grid. \hey{this Xfoot is not used anywhere in the subsequent discussion. Why do we need this? we can just say (x_{foot}, y_{foot}, z_{foot}) denote the co-ordinates of the lowest point of on feet of the human avatar mesh and move on?}

    We use a sliding volume approach over $V(x,y,z)$ on layers from $z=\hat{h}_{floor\_vox}$ to $z=\hat{h}_{floor\_vox}+h_{human\_vox}$, where $h_{human\_vox}$ is the height of the voxelized human avatar. Each volume in the sliding volume is equal to the size \hey{what do you mean by size? is it max cubioid dimension needed to fit the human when performing pointing? Can the cuboid be rotated in the grid?} of the human avatar voxel grid. Over this volume, we use the human voxel grid as a mask to check if there is exactly enough space to fit the voxel grid of the human in that sliding volume of $V$. Given a volume $(i,j,\hat{h}_{floor\_vox})$ to $(i+x_{max}, j+y_{max}, \hat{h}_{floor\_vox}+h_{human\_vox})$, \hey{how do you find xmax,ymax,zmax? is it the diagonal of the base rectangle of the cuboidal volume?}such that 
    \begin{dmath}\label{eq: occ_points}
    \sum_{x=0}^{x_{max}}\sum_{y=0}^{y_{max}}\sum_{z=0}^{z_{max}}H(x,y,z)=\sum_{x=0}^{x_{max}}\sum_{y=0}^{y_{max}}\sum_{z=0}^{z_{max}}{H(x,y,z) \times V_1(i+x,j+y,k+z)}
    \end{dmath}
    \hey{what is this equation? there is H(x,y,z) on both sides of the equation and there is a `such that' condition for what?. Or is it a condition that needs to be satisfied to day that a given volume is totally clear? Symbol H is already used for human voxel grid.}

    We define a function $F_{clear\_space}: \mathbb{R}^2 \rightarrow \{1,0\}$ such that
    \begin{equation}
        F(i,j)= 
        \begin{cases}
            1,&             \text{if } (i,j,k) \text{ satisfies \ref{eq: occ_points}}\\
            0,              & \text{otherwise}
        \end{cases}
    \end{equation}

It is important to note that after the rotation, the re-oriented human avatar may collide with the object of interest if it is positioned too close to an occupied boundary in $F_{clear\_space}$. Thus, we increase the border widths in $F_{clear\_space}$ by $10$ voxels. We store $(i,j,\hat{h}_{floor\_vox}+h_{human\_vox})$ in the set $O_{no\_collide}$ if $F_{clear\_space}=1$.
    
\noindpar{Grid visibility search: } Visibility between two points can be determined without directly checking for a line of sight, particularly in grid-based environments \cite{buildingvis}. A path-counting algorithm has been used in 2D to calculate visibility scores for each grid cell, as explored in \cite{gridwalk}. We extend this approach to 3D environments. Given $V_2$, we compute a visibility score grid, denoted as $S(\mathbb{N}^3 \rightarrow \mathbb{R})$, where $S$ is defined as:

\begin{dmath}    
%    S(x,y,z) = V_2(x,y,z) \times\frac{x \times S(x-1,y,z) + y \times S(x,y-1,z) + z \times S(x,y,z-1)}{x+y+z} 
    S(x,y,z) = (\frac{x \times S(x-1,y,z)}{x+y+z} + \frac{y \times S(x,y-1,z)}{x+y+z} + \frac{z \times S(x,y,z-1)}{x+y+z} ) \times V_2(x,y,z)
\end{dmath}

We then obtain $S'(\mathbb{N}^3 \rightarrow \{1,0\})$ a thresholded version of $S$ as follows:
\begin{equation}
        S'(x,y,z)= 
\begin{cases}
    1,&             \text{if } S(x,y,z)\geq0.33\\
    0,              & \text{otherwise}
\end{cases}
\end{equation}
$S'$ gives us a good approximation for all the visible regions. We define the set of all the coordinates where $S'=1$ as the \emph{region of visibility}. Figure \ref{fig:grid_visibility} shows an example of such a region of visibility. A threshold of 0.33 was chosen empirically.

\noindpar{Computing the final transformation matrix: }     
%     \par{\st{We then iterate over the entire scene with iterating over the coordinates $\vec{v}_{iter}=(i,j,k)$. We iterate only in the $XY$-plane; We set $k=max(Z_{floor}, Z_{foot})$. $\vec{v}_{iter}$ represents the point on the floor of the scene where one of the bottom corners of the voxel grid made from human avatar mesh will be placed. This ensures that the new augmented position of the human avatar is always above the floor. Additionally, we reduce the number of computations needed by confining the search space from 3D grid traversal to 2D grid traversal by limiting the exploration to a single plane. }
%     \par{\st{For each iteration we consider a cuboidal volume $E$ from $(i,j,k)$ to $(i+x_{max}, j+y_{max}, k+z_{max})$. Here, $x_{max},y_{max},z_{max}$ are the maximum bounds of the human avatar voxel grid. For every iteration, we check if the following equality condition is satisfied:}}
% \begin{dmath}\label{eq: occ_points}
% \sum_{x=0}^{x_{max}}\sum_{y=0}^{y_{max}}\sum_{z=0}^{z_{max}}H(x,y,z)=\sum_{x=0}^{x_{max}}\sum_{y=0}^{y_{max}}\sum_{z=0}^{z_{max}}{H(x,y,z) \times V_1(i+x,j+y,k+z)
% }
% \end{dmath}


% \par{\st{Here, $H, V_1$ are the voxel grid formed from the human avatar mesh and the voxel grid formed from the original scene mesh, respectively, as defined earlier.} 
% }

% \par{
% \st{Intuitively, the equation} (\ref{eq: occ_points}) \st{creates a mask of the shape of the human avatar for the cuboidal space $E$ and queries if the sum of the cells resultant is equal to the sum of the cells of the human mask, i.e., it checks if the human avatar can fit in the space $E$. Since we are checking for occupancy, we must also restrict the human avatar from occupying the voxels occupied by the 'object of interest.' For this reason, we need an 'un-occupancy grid' for the entire un-altered original scene. Thus, we use $V_1$ here.}
% }

For the coordinate $(i,j,k)$ in the voxel grid, the \textit{boundary} condition can be checked by querying the value $B(i,j,k)$. 
If it is $1$, then \textit{boundary} condition is satisfied. 
Similarly, if $(i,j,k) \in O_{no\_collide}$, then, $(i,j,k)$ also satisfies the \textit{overlap} condition. 
If $S'(x,y,z)=1$ then $(i,j,k)$ also satisfies the \textit{ line-of-sight} condition. 
Thus the aim is to new_data_2.append(img)collect all such points. \hey{what is this?} 
These are the potential points where the human point cloud could be augmented. 
We place these points in a container $C_{initial\_samples}.$
 
% \par{
% \st{Given the coordinate of the shoulder in the human voxel grid $\vec{v}_{shoulder\_hum\_vox}=(x_s,y_s,z_s)$, for each coordinate $\vec{v}_{iter}$ %, the coordinate of the shoulder such that 
% the human avatar is imputed at $\vec{v}_{iter}$ is $(x_s+i,y_s+j,z_s+k)$. We query $S'(x_s+i,y_s+j,z_s+k)$, and if this value is 1 then condition \#3 is satisfied. %\am{ a run-on sentence, needs to be modified}
% Essentially, the aim is to collect all the grid coordinates 
% $\vec{v}_{sample\_point}=(x_s+i,y_s+j,z_s+k)$ }}. 

We use the gesturing shoulder of the human avatar as a pivot of rotation to point toward the object of interest. It is sufficient to fit the shoulder in the region of visibility since having the pivot inside the region of visibility ensures that after rotation, the entire gesture (in our case, the hand) lies inside the region of visibility.
%}

We construct a set $C_{final\_samples}$ from the points that satisfy the above equation. \hey{when there are multiple vacant spaces that satisfy the three conditions, how does Imputer choose the position of the avatar?}
After finding the coordinates mentioned in the condition above, we calculate simple Euclidean transforms to move the human from its original position to the desired coordinate and then rotate the human in place. 

We have the coordinates of 4 points, each of which we convert to homogeneous coordinates: 
\begin{enumerate}
    \item The coordinates of the shoulder of the human $\vec{S}=[S_x, S_y, S_z, 1]^T$.
    \item The coordinates of the tip of the pointing gesture $\vec{P}=[P_x, P_y, P_z, 1]^T$.
    \item The coordinates of the desired destination for the human pointcloud $\vec{D}=[D_x, D_y, D_z, 1]^T$ and
    \item The coordinates of the centroid of the bounding box of the 'object of interest' $\vec{B}=[B_x, B_y, B_z, 1]^T$.
\end{enumerate}

We define the translation matrix $\mathbf{M_{t}}$ that moves the human from its current position to the destination as follows:
\begin{equation}
    \mathbf{M_{t}} = \begin{bmatrix}
                                    1 & 0 & 0 & D_x-S_x\\
                                    0 & 1 & 0 & D_y-S_y\\
                                    0 & 0 & 1 & D_z-S_y\\
                                    0 & 0 & 0 & 1
                                    \end{bmatrix}
\end{equation}

We compute $\vec{S'} = \mathbf{M_t}\cdot\ \vec{S}$ and $\vec{P'} = \mathbf{M_t}\cdot\ \vec{P}$ and convert each of the obtained vectors back to cartesian coordinate. We note that $\vec{S'}=\vec{D}$. 

From here, we compute a rotation matrix that, when applied to $\vec{E} = \vec{P'} - \vec{S'}$, aligns the vector with $\vec{F} = \vec{B} - \vec{S'}$. We first get the unit vectors in each direction as $\hat{E}=\frac{\vec{E}}{|\vec{E}|}$ and $\hat{F}=\frac{\vec{F}}{|\vec{F}|}$.
We then define the rotation matrix $\mathbf{M_r}$ as 
\begin{equation}
    \mathbf{M_r}=\mathbf{I} + \mathbf{V} + (\frac{1-\hat{E}^T\cdot \hat{F} \hat{}}{|\vec{V}|^2})( \mathbf{V}^T\cdot\mathbf{V})
\end{equation}
Where $\vec{V} = \hat{E} \times \hat{F} $. Let $\vec{V}=[V_x, V_y, V_z]$
\begin{equation}
    \mathbf{V} = \begin{bmatrix}
                                    0 & -V_z & -V_y \\
                                    V_z & 0 & -V_x \\
                                    V_y & V_x & 0
                    \end{bmatrix}
\end{equation}
Note that $\mathbf{M_r}$ is a $3\times3$ matrix, and that this rotational matrix would rotate the human avatar correctly, if the pivot, i.e. the shoulder, was placed at the origin. To take the shift of the shoulder into account after translation, we use the following final $4\times4$ rotation in homogeneous coordinate:
\begin{equation}
    \mathbf{M_R} = \begin{bmatrix}
    \mathbf{M_r} & \vec{S}-\mathbf{M_r}\vec{S}\\
    0 & 1
    \end{bmatrix}
\end{equation}
This can be easily obtained by the following matrix multiplications.
\begin{equation}
    \mathbf{M_R} = \begin{bmatrix}
    \mathbf{I_{3\times3}} & \vec{S}\\
    0 & 1
    \end{bmatrix}
    \begin{bmatrix}
    \mathbf{M_r} & \vec{0}\\
    0 & 1
    \end{bmatrix}
    \begin{bmatrix}
    \mathbf{I_{3\times3}} & -\vec{S}\\
    0 & 1
    \end{bmatrix}
\end{equation}
Where $\vec{0}$ represents a 3 dimensional vector of length $0$ and $\mathbf{I_{3\times3}}$ represents a $3\times3$ identity matrix.
\par We then store the final matrix $\mathbf{M} = \mathbf{M_R} \cdot \mathbf{M_t}$.

When loading the dataset, we load the scene and the human pointcloud seperately. We then add a rotational jitter of  range $N_{jitter} = 9^{\circ}$ to simulate measurement errors while capturing the human. \hey{reframe this}



Figure \ref{fig:success_impute} shows the human avatar placed in a 3D scene, which is marked by a red box, pointing towards the target object marked by a green box.
\fi

\subsection{Referring Expression (Re)Generation:} We now use Gemini~\cite{gemini} to augment the referring expression. For each data point in the ScanRefer \cite{chen2020scanrefer} dataset, we ask the model to generate 3 referring expressions. %As input, we pass 3 images, which represent 3 views of the scene, the top view, the human perspective view, and the side view following the methodology of~\cite{caesar}.
We prompt the model to generate the referring expression based on context from a small paragraph of text given with a language prompt to Gemini (Included in the supplementary materials).

\section{\texorpdfstring{\names} \ : A Gesture-enhanced 3D Visual Grounding Model}

% \begin{figure*}[!htb]
%     \centering
%     \begin{minipage}{0.25\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{Fig/human_pcds.png}
%         \caption{Example human models used in \aug framework}
%         \label{fig:pcds}
%     \end{minipage}%
%     \hfill
%     \begin{minipage}{0.75\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{Fig/architecture3.png}
%         \caption{Proposed architecture of \names.}
%         \label{fig:architecture}
%     \end{minipage}
% \end{figure*}

% \begin{figure*}[!htb]
%     \centering
%     % First figure (20% width)
%     \begin{minipage}{0.15\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{Fig/human_pcds.png}
%         \caption{Example human models used in \aug framework}
%         \label{fig:pcds}
%     \end{minipage}%
%     \hfill
%     % Second figure (30% width)
%     \begin{minipage}{0.7\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{Fig/architecture.png}
%         \caption{Proposed architecture of \names.}
%         \label{fig:architecture}
%     \end{minipage}%
%     \hfill
%     % Subfigures 2x2 grid (50% width total, each subfigure takes up 50% of this 50%)
%     \begin{minipage}{0.15\textwidth}
%         \centering
%         \begin{subfigure}{0.49\textwidth}
%             \centering
%             \includegraphics[width=\linewidth]{Fig/imputer_figs/visibility_scores.png}
%             \caption{Correctly placed human (Red box) pointing to object (green box).}
%             \label{fig:subfigure1}
%         \end{subfigure}%
%         \hfill
%         \begin{subfigure}{0.49\textwidth}
%             \centering
%             \includegraphics[width=\linewidth]{Fig/imputer_figs/visibility_scores.png}
%             \caption{Subfigure 2}
%             \label{fig:subfigure2}
%         \end{subfigure}

%         \vspace{1em} % Space between subfigures

%         \begin{subfigure}{0.49\textwidth}
%             \centering
%             \includegraphics[width=\linewidth]{Fig/imputer_figs/visibility_scores.png}
%             \caption{Subfigure 3}
%             \label{fig:subfigure3}
%         \end{subfigure}%
%         \hfill
%         \begin{subfigure}{0.49\textwidth}
%             \centering
%             \includegraphics[width=\linewidth]{Fig/imputer_figs/visibility_scores.png}
%             \caption{Subfigure 4}
%             \label{fig:subfigure4}
%         \end{subfigure}
%     \end{minipage}
% \end{figure*}

% \begin{figure}[!htb]
%     \centering
%     \begin{subfigure}{.1\textwidth}
%         \centering
% \includegraphics[width=\linewidth]{Fig/imputer_figs/successful_imputation2.png}
%     \caption{Illustration of a correctly placed human (Red box) pointing to object (green box).}
%     \label{fig:success_impute}
%     \end{subfigure}%
%     \hfill
%     \begin{subfigure}{0.1\textwidth}
%         \centering
%     \includegraphics[width=\linewidth]{Fig/imputer_figs/contour.png}
%     \caption{Contour formed by the boundary of a scene in the voxel grid.}
%     \label{fig:contour}
%     \end{subfigure}
% \hfill
%         \begin{subfigure}{0.1\textwidth}
%         \centering
%     \includegraphics[width=\linewidth]{Fig/imputer_figs/countour_filled.png}
%     \caption{Determining the bounds of the scene by filling contours in the voxel grid.}
%     \label{fig:contour_filled}
%     \end{subfigure}
%     \hfill
%             \begin{subfigure}{0.1\textwidth}
%         \centering
%     \includegraphics[width=\linewidth]{Fig/imputer_figs/visibility_scores.png}
%     \caption{Grid visibility search to identify the line-of-sight to human from target object.}
%     \label{fig:grid_visibility}
%     \end{subfigure}
%     \vspace{-0.1in}
%     \caption{Intermediate steps from \aug framework}
% \end{figure}
\begin{figure}
    \centering
    \begin{minipage}{0.18\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Fig/human_pcds.png}
        \caption{Sample human models}
        \label{fig:pcds1}        
    \end{minipage}
    \hfill
    \begin{minipage}{0.8\linewidth}
        \centering

        % \hfill
        \begin{subfigure}{0.23\textwidth}
            \centering
            \includegraphics[width=\linewidth]{Fig/imputer_figs/contour.png}
            \caption{Contour formed by scene boundary.}
            \label{fig:contour}
        \end{subfigure}%
        \hfill
        \begin{subfigure}{0.23\textwidth}
            \centering
            \includegraphics[width=\linewidth]{Fig/imputer_figs/countour_filled.png}
            \caption{Filling contours for bounds.}
            \label{fig:contour_filled}
        \end{subfigure}%
        \hfill
        \begin{subfigure}{0.23\textwidth}
            \centering
            \includegraphics[width=\linewidth]{Fig/imputer_figs/visibility_scores.png}
            \caption{Grid visibility search for line-of-sight.}
            \label{fig:grid_visibility}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.23\textwidth}
            \centering
            \includegraphics[width=\linewidth]{Fig/imputer_figs/successful_imputation2.png}
            \caption{Correctly placed human pointing to object.}
            \label{fig:success_impute}
        \end{subfigure}%
        \caption{Intermediate steps from \aug framework}
    \end{minipage}
\end{figure}



\begin{figure}
    \centering
    \includegraphics[width=0.99\linewidth]{Fig/architecture4.png}
    \caption{Proposed architecture of \namess.}
    \label{fig:architecture}
    \vspace{-0.2in}
\end{figure}
We present \namess, a novel approach to gesture-enhanced 3D visual grounding that integrates human localization, language understanding, and gestural reasoning to identify the 3D bounding box of the target object within a single feed-forward network. To effectively combine gestural and linguistic cues, we introduce a mutli-stage fusion strategy that employs both early and late fusion within the same DNN. Our proposed approach is shown in the Figure~\ref{fig:architecture}. We now highlight the key components of \namess

\subsubsection{\textbf{Vision Module}\label{sec:vismod}} We first encode the point cloud features using a PointGroup detector \cite{pointgroup}. PointGroup, being a standard object detector for 3D point clouds $P\in \mathbb{R}^{N\times C}$, returns both the visual features and all the objects in the scene. Here, 
$N$ is the number of points in the PointCloud and $C$ is the number of channels per point, including the 3D coordinate, the per-point surface normal vector and the color of the point.\\
We use the following outputs from the PointGroup Detector for further processing:
\begin{enumerate}
    \item Semantic Features ($F_s \in \mathbb{R}^{N\times32}$)
    \item Semantic Scores ($S_s \in \mathbb{R}^{N\times N_c}$) where $N_c$ is the number of classes in the dataset.
    \item Proposal Features ($F^{3D}_p \in \mathbb{R}^{M\times 32}$) where $M$ is the number of proposals.
    \item Proposal Scores ($S_p \in \mathbb{R}^{M}$) These are essentially the instance/objectness scores for each proposal.
\end{enumerate}
We use $F_s$ and $S_s$ for Gesture Inference as given in Section~\ref{sec:GesEnc}, while $S_p$ is used to find proposals and $F^{3D}_p$ is passed ahead to be used as 3D visual features.

For each proposal $P$, we then render the object from 3 different views as images. The images are then passed into a CLIP \cite{clip} image encoder. The output is then used as 2D features ($F^{2D}_p \in \mathbb{R}^{M \times 128}$) for each proposal. $F^{3D}_p$ and $F^{2D}_p$ are then concatenated into joint visual features and passed through a 1D convolution to get $F_{v} \in \mathbb{R}^{M \times 128}$
%PointGroup uses a U-Net based on a sparse-voxelized version of the input pointcloud module to compute semantic features. They project these voxel-based features back to the pointcloud domain through a voxel-point map computed during the voxelization process. PointGroup uses these semantic features to calculate semantic scores. We store these semantic scores and features to infer gesture-based information mentioned in \ref{sec:GesEnc}.
%They also have an 'offset prediction head' that they use clustering points into instances. They introduce a clustering algorithm and use it on the set of original coordinates from the pointcloud and also on a the coordinates of the pointcloud after offsetting them using the output of the 'offset prediction head'. They then pass then pass the voxelized version of each of the proposals.

\subsubsection{\textbf{Language Feature Encoder }} For language features, we use CLIP language features \cite{clip} for getting sentence level and token level feature embeddings. We define our sentence features as $F_{l,s} \in \mathbb{R}^{128}$ and word features as $F_{l,t} \in \mathbb{R}^{N_{token}\times 128}$, for an $N_{token}$ token long sequence.

\subsubsection{\textbf{Gesture Feature Encoder }\label{sec:GesEnc}} 

% The objective of this module is to facilitate gestural reasoning for the human segments identified from the region proposals generated by the PointGroup detector. To achieve this, we efficiently reuse the semantic features, denoted as $F_s$, which are computed in Section \ref{sec:vismod}. Specifically, for a given human segment $P_{hum} \in P$, which consists of $N_{hum}$ points, we extract a corresponding subset of semantic features, $F_{s,hum} \in F_s$, comprising $N_{hum}$ vectors. Given an expected number of human joints, $N_j \in \mathbb{N}$, the semantic feature subset $F_{s,hum}$ is passed through a point-wise MLP, inspired by PointNet \cite{Pointnet}, to produce an output $W_{hum} \in \mathbb{R}^{N_{hum} \times N_j}$. The joint coordinates $J \in \mathbb{R}^{N_j \times 3}$ are then derived from $W_{hum}$ as follows:

The objective of this module is to enable gestural reasoning for human segments identified from region proposals generated by the PointGroup detector. To accomplish this, we employ the following components within the Gesture Feature Encoder.

\begin{enumerate}[leftmargin=*]
    \item \textbf{Gesture Encoder: } We begin by using a Gesture Encoder to compute the features of the pointing human. As input, we leverage semantic features, represented by $F_s$, which are computed in the vision module. Specifically, for a given human segment $P_{hum} \in P$, comprising $N_{hum}$ points, we extract a corresponding subset of semantic features, $F_{s,hum} \subset F_s$, consisting of $N_{hum}$ vectors. Given an anticipated number of human joints, $N_j \in \mathbb{N}$, the semantic feature subset $F_{s,hum}$ is processed through a point-wise MLP inspired by PointNet \cite{Pointnet}, resulting in an output $W_{hum} \in \mathbb{R}^{N_{hum} \times N_j}$. Inspired from Point2Skeleton \cite{Point2Skeleton} the joint coordinates $J \in \mathbb{R}^{N_j \times 3}$ are then computed from $W_{hum}$ as follows:
    \begin{equation}
        J = Softmax(W_{hum}^T) \times P_{hum}
    \end{equation}
    We also obtain the initial joint-based features $F_{j, init} \in \mathbb{R}^{N_j,32}$ as follows:
    \begin{equation}
        F_{j,init} = Softmax(W_{hum}^T) \times F_{s,hum}
    \end{equation}
    \item \textbf{Joint-Wise MLP: } Next, we concatenate the location of each joint with its corresponding feature to form $F_{j,init}$. This concatenated feature is then processed by the proposed Joint-wise MLP, which consists of $N_{layers}$ layers. In this configuration, the MLP processes each feature vector independently for each joint. Let $M_i$ represent the $i$-th layer of the MLP, and let $P_{j,i}$ denote its output for the $j$\textsuperscript{th} joint. This module produces the following outputs:
    \begin{multline}
        F_{j,final} = P_{j,N_{layers}}~; ~where ~P_{j,i} = M_{i}(P_{j,i-1}) \\ and ~P_{j,1} = M_{1}(F_{j,init})
    \end{multline}
    %where 
    %\begin{equation}
    %    P_{j,i} = M_{i}(P_{j,i-1})
    %\end{equation}
    %and
   % \begin{equation}
    %    P_{j,1} = M_{1}(F_{j,init})
    %\end{equation}
    \begin{equation}
        F_{j,aggregate} = concatenate_{i=0}^{i=N_{layers}}{\sum_{j=0}^{N_{j}}{P_{j,i}}}
    \end{equation}
    Here $N_j$ is the number of joints specified in SMPL
    
\end{enumerate}

% We add a human key point detector module to our dataset. The task of this module is similar to 3D joint detection models. We efficiently re-use the semantic features $F_s$ calculated in \ref{sec:vismod}. We use method similar to the one proposed in Point2Skeleton \cite{Point2Skeleton}. Given a human segment $P_{hum}\in P$ with $N_{hum}$ number of points, a semantic feature subset $F_{s,hum}\in F_s$ with $N_{hum}$ number of vectors, and a expected number of joints in human $N_j \in \mathbb{N}$, we pass $F_{s,hum}$ through a point-wise MLP similar to Pointnet\cite{Pointnet} to get an output $W_{hum} \in \mathbb{R}^{N_{hum} \times N_j}$. From $W_{hum}$ we get the coordinates of joints $J \in \mathbb{R}^{N_j\times 3}$ as follows:

% \subsubsection{\textbf{Joint-Wise MLP Module }\label{sec:JointWiseMLP}} 
% We concatenate the location and its corresponding feature for each joint to form $F_{j,init}$. This concatenated feature is then passed through a ``Joint-wise MLP'' consisting of $N_{layers}$ layers. In this setup, the MLP processes each feature vector independently for each joint. Let $M_i$ represent the $i$-th layer of the MLP, and $P_i$ denote its output. This module produce the following outputs:
% \begin{equation}
%     F_{j,final} = P_{N_{layers}}
% \end{equation}
% Where
% \begin{equation}
%     P_{i} = M_{i-1}(P_{i-1})
% \end{equation}
% and
% \begin{equation}
%     P_{1} = M_{0}(F_{j,init})
% \end{equation}
% \begin{equation}
%     F_{j,aggregate} = concatenate_{i=0}^{i=N_{layers}}{\sum_{k=0}^{N_{j}}{P_i}}
% \end{equation}

%\subsubsection{\textbf{Language and Vision Feature Fusion: }}
%\dw{Explain what the output of this is, is it the confidence value %for each boudning box?}
%\dw{Explain with equations}


% We use the geometric-distance \textbf{(or L2 loss.. Gotta check)} between the prediction and label coordinates to regress for the final points.
\subsubsection{\textbf{Early Fusion of Gestural and Language Features }}

Our approach hinges on a hybrid fusion of language and gestural features, combining early and late fusion techniques. In the proposed early fusion module, we utilize $F_{j, final} \in \mathbb{R}^{N_j \times 128}$, treating these features similarly to word embeddings from the Language Feature encoder. The intuition behind this is that both human gesture features and language features act as clues or aids in identifying the correct object within a scene, making them suitable for similar treatment. Initially, we pass $F_{j, final}$ through two self-attention layers, after which they are concatenated with $F_{l, t}$ to form $F_{clue} \in \mathbb{R}^{(N_{token} + N_j) \times 128}$.

% Finally, we propose a "Human-Language Processing" module. Through our Joint-Wise MLP proposed in Section \ref{sec:JointWiseMLP} we ensure that $F_{j, final}\in \mathbb{R}^{N_j\times 128}$. We propose to treat these features similar to the word embedding from the Language Feature encoder. The intuitive reasoning for this is that both, the human gesture features and the language features serve as a clue/assistance, to pointing out the correct object in the scene, and thus could be treated similarly. We first pass $F_{j,final}$ through 2 self attention layers, after which they are concatenated with $F_{l,t}$ to get $F_{clue} \in \mathbb{R}^{(N_{token}+N_j)\times 128}$

\subsubsection{\textbf{Fusion Module}}
We employ the same transformer-based fusion module as M3DRef-CLIP~\cite{m3drefclip} to integrate object features with the human-language embeddings $F_{clue}$, generating confidence scores ($S_{conf} \in \mathbb{R}^{M}$) for each proposal. This module consists of two self-attention and two cross-attention blocks, where the object features sequentially pass through the self-attention and cross-attention blocks. In the cross-attention blocks, $F_{clue}$ is used as the key-value pairs.

% \artharv{Needs to change slightly}
\subsubsection{\textbf{Late Fusion of Gestural and Language Scores }}

The output from the fusion module provides confidence scores for each object proposal, allowing the selection of the target object based on the highest score. To further refine this process, we introduce an additional constraint by implementing a late fusion approach that adaptively biases confidence scores in the direction of pointing. Specifically, we compute a pointer biasing score, denoted as $S_b \in \mathbb{R}^{M}$, and adaptively add it to $S_{conf}$ to guide predictions toward points that are angularly closer to the pointing direction.
To achieve this, we first extract the shoulder and fingertip points from $O_{human}$. Let these points be represented by $\vec{v_1} \in \mathbb{R}^{3}$ and $\vec{v_2} \in \mathbb{R}^{3}$, respectively. The center coordinates of a predicted bounding box $B$ are represented by $\vec{v_3} \in \mathbb{R}^{3}$.
The pointer bias score $S_b$ is defined as follows:
\begin{equation} \label{eqn:Pointerbiasingeqn}
    S_b = \frac{(\vec{v_2}-\vec{v_1})\cdot (\vec{v_3}-\vec{v_1})}{||((\vec{v_2}-\vec{v_1}))||\cdot||((\vec{v_3}-\vec{v_1}))||}
\end{equation}

We calculate $S_{b,left} \in \mathbb{R}^{M}$ and $S_{b,right} \in \mathbb{R}^{M}$ using the equation \ref{eqn:Pointerbiasingeqn} for both left and right hand respectively.

% We also calculate $W_{score\_agg} \in \mathbb{R}^2$ as follows:
% \begin{equation}
%     W_{score\_agg} = SoftMax(MLP2(F_{j,aggregate}))
% \end{equation}

Intuitively, humans may use either the left or right hand for pointing. To classify the pointing hand used, we employ a classification head that takes $F_{j,aggregate}$ as input to learn $W_{lr_agg} \in \mathbb{R}^{2}$ as follows.
\begin{equation}
    W_{lr\_agg} = Softmax(MLP1(F_{j,aggregate}))
\end{equation}
With the calculated $W_{lr\_agg}$, we compute the final biasing score $S_{b,final}$ as follows. \hey{may need to explain why we used soft probability instead of hard argmax here}
% \begin{equation}
%         S_{b,final}= 
% \begin{cases}
%     S_{b,left}&             \text{if } argmax(W_{lr\_agg})=0\\
%     S_{b,right}              & \text{otherwise}
% \end{cases}
% \end{equation}
\begin{equation}
    S_{b,final} = W_{lr\_agg}^0*S_{b,left} + W_{lr\_agg}^1*S_{b,right}
\end{equation}
With the computation of $S_{b,final}$ from the pointer biasing score and $S_{conf}$ from the fusion module, we now have two sets of object scores. To obtain the final object scores, we propose using an additional probabilistic head, denoted as $W_{score_agg} \in \mathbb{R}^{2}$, which adaptively aggregates scores from the two branches. This aggregation is computed as follows.
\begin{equation}
    W_{score\_agg} = SoftMax(MLP2(F_{j,aggregate}))
\end{equation}
The final object scores are then obtained using the following equation and the target object is identified by the object proposal with the highest $S_{conf,final}$.
\begin{equation}
    S_{conf,final} = W_{score\_agg}^0*S_{conf} + W_{score\_agg}^1*S_{b,final}
\end{equation}
% we aggregate between $S_{b,left}$ and $S_{b,right}$ to get $S_b$. While using $W_{score\_agg}$ we aggregate between $S_b$ and $S_{conf}$ to get the final biased confidence scores.  $S_b$ can be interpreted as the expected biasing score where the probabilistic event is choosing the hand that is being used for pointing. While the $W_{score\_agg}$ can be interpreted as the confidence of the model over each type of prediction, that from the so called "early-fusion" of the human information or that from naive Angular Distance-based Biasing.
% Intuitively, human may use either the left or the right hand for pointing. Thus, $W_{lr\_agg}$ we aggregate between $S_{b,left}$ and $S_{b,right}$ to get $S_b$. While using $W_{score\_agg}$ we aggregate between $S_b$ and $S_{conf}$ to get the final biased confidence scores.  $S_b$ can be interpreted as the expected biasing score where the probabilistic event is choosing the hand that is being used for pointing. While the $W_{score\_agg}$ can be interpreted as the confidence of the model over each type of prediction, that from the so called "early-fusion" of the human information or that from naive Angular Distance-based Biasing.
% \par We use the $F_{j, aggregate}$ define in \ref{sec:JointWiseMLP}, which represents the "overall features" of the human model and pass it through 2 seperate MLPs to predict 2 scores. The so called "LR" score, $\vec{S_{lr}} \in \mathbb{R}^2$ which tries to predict which pointing hand is used left or right and the so called "biaser score" $\vec{S_{biaser}} \in \mathbb{R}^{2}$ which determines the weights that need to be given to $S_b$ and $S_{conf}$ for each object.
% The Final score $S_f\in \mathbb{R^M}$ is given as 
% \artharv{Needs to change slightly}

\subsubsection{\textbf{Loss Function: }}
Proposed loss function comprises of the following terms. \\
\textbf{Object Detection Losses:}
\begin{enumerate}
    \item Cross-entropy loss for supervising per-point semantic class prediction called the Semantic Loss, $L_{semantic}$. 
    \item L1 loss for supervising per-point offset vector towards object centers (useful for instance segmentation), called the Offset Norm Loss, $L_{offset\_norm}$.
    \item A directional loss formed as a mean of minus cosine similarities to constrain the direction of per-point offset vectors called the Offset Direction Loss, $L_{offset\_dir}$.
    \item A binary cross-entropy loss for supervising per-point objectness confidence score is called the Score Loss, $L_{score}$.
    \end{enumerate}
\textbf{Reference Understanding Losses:}
\begin{enumerate}[start=5]
    \item The Reference Loss, $L_{ref}$, is a multi-class cross-entropy loss to classify the object that the referring expressions refer to.
    \item A symmetric contrastive loss, $L_{contrastive}$ between sentence features and the visual features to aid training. 
\end{enumerate}
\textbf{Human Localization Loss:}
\begin{enumerate}[start=7]
    \item A human joint prediction loss to regress over the joints of the augmented human defined as'
 \begin{dmath*}
     L_{hum} = \sum_{joint\in joints} {||\vec{v}_{joint, pred}-\vec{v}_{joint, gt}||}
\end{dmath*}
where joints is the set of all the joints of the human defined in the human avatar skeleton.
    \item Finally, a classification loss $L_{lr}$ over $W_{lr\_agg}$ to classify the gesture as left handed or right handed.
\end{enumerate}

\subsubsection{\textbf{Training Details: }} We utilize an iterative training approach where we first train the PointGroup detector and gesture feature encoder for 20 epochs with a learning rate of 0.00005 with cosine annealing, using the Adam optimizer. At this step, loss term $L_{semantic}$, $L_{offset\_norm}$, $L_{offset\_dir}$, $L_{score}$ and $L_{hum}$ are enabled for optimization.

Subsequently, we freeze the PointGroup detector and the gesture feature encoder and only enable the matching module with the loss terms $L_{ref}$ and $L_{contrastive}$ enabled for optimization. This step trains the comprehension module to comprehend verbal instruction.
%\artharv{Note: $L_{contrastive}$ doesn't get trained since for CLIP model is frozen both in pertaining and main-training. Although it will be used in ablation studies. IDK how we should denote this. There is probably only 1 MLP that gets trained. The 1 that combines $F^{3D}_vis and F^{2D}_vis$ }


% \begin{figure}[!htb]
%     \centering
%     \begin{subfigure}{0.48\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{Fig/imputer_figs/successful_imputation2.png}
%         \caption{Correctly placed human (Red box) pointing to object (green box).}
%         \label{fig:success_impute}
%     \end{subfigure}%
%     \hfill
%     \begin{subfigure}{0.48\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{Fig/imputer_figs/contour.png}
%         \caption{Contour formed by the boundary of a scene in the voxel grid.}
%         \label{fig:contour}
%     \end{subfigure}
%     \vskip\baselineskip
%     \begin{subfigure}{0.48\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{Fig/imputer_figs/countour_filled.png}
%         \caption{Filling contours in the voxel grid to determine scene bounds.}
%         \label{fig:contour_filled}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.48\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{Fig/imputer_figs/visibility_scores.png}
%         \caption{Grid visibility search for line-of-sight to human from target object.}
%         \label{fig:grid_visibility}
%     \end{subfigure}
%     \caption{Intermediate steps from \aug framework}
%     \label{fig:2x2_grid_single_column}
%     \vspace{-0.1in}
% \end{figure}



% \begin{figure}[!htb]
%     \centering
%     \begin{subfigure}{.1\textwidth}
%         \centering
% \includegraphics[width=\linewidth]{Fig/imputer_figs/successful_imputation2.png}
%     \caption{Illustration of a correctly placed human (Red box) pointing to object (green box).}
%     \label{fig:success_impute}
%     \end{subfigure}%
%     \hfill
%     \begin{subfigure}{0.1\textwidth}
%         \centering
%     \includegraphics[width=\linewidth]{Fig/imputer_figs/contour.png}
%     \caption{Contour formed by the boundary of a scene in the voxel grid.}
%     \label{fig:contour}
%     \end{subfigure}
% \hfill
%         \begin{subfigure}{0.1\textwidth}
%         \centering
%     \includegraphics[width=\linewidth]{Fig/imputer_figs/countour_filled.png}
%     \caption{Determining the bounds of the scene by filling contours in the voxel grid.}
%     \label{fig:contour_filled}
%     \end{subfigure}
%     \hfill
%             \begin{subfigure}{0.1\textwidth}
%         \centering
%     \includegraphics[width=\linewidth]{Fig/imputer_figs/visibility_scores.png}
%     \caption{Grid visibility search to identify the line-of-sight to human from target object.}
%     \label{fig:grid_visibility}
%     \end{subfigure}
%     \vspace{-0.1in}
%     \caption{Intermediate steps from \aug framework}
% \end{figure}


% \begin{figure}
%     \centering
%     \includegraphics[scale=0.2]{samples/Fig/imputer_figs/successful_imputation.png}
%     \caption{Illustration of a correctly placed human (in red bounding box pointing to an object (green bounding box)}
%     \label{fig:succimp}
% \end{figure}

% \begin{figure}[H]
%     \centering
%      \begin{subfigure}[t]{0.2\textwidth}
%          \includegraphics[width=\textwidth]{samples/Fig/imputer_figs/contour.png}
%          \caption{Contour formed by boundary of $scene0000\_00$ from the ScanNet dataset \cite{scannet}}
%          \label{fig:contour}
%          \hspace{1em}%
%     \end{subfigure}
%     \hspace{0.05\textwidth}
%     \begin{subfigure}[t]{0.2\textwidth}
%          \includegraphics[width=\textwidth]{sample/Fig/imputer_figs/countour_filled.png}
%          \caption{The contour in Figure \ref{fig:contour} filled-up to obtain the entirety of inner space}
%          \label{fig:contour_filled}
%     \end{subfigure}
%     \caption{}
% \end{figure}

% \begin{figure}[H]

%     \centering
%     \includegraphics[scale=0.3]{samples/Fig/imputer_figs/visibility_scores.png}
    
%     \caption{Figure showing the visibility score region for the object in the green bounding box.
% For ease of understanding, each point in the visibility region appears with the probability equivalent to its visibility score. This means that the visibility score of a region can be modeled by its density. The ripple red is highlighted to depict that the visibility region models light originating from the center of the object of interest (inside the green bounding box) to the outside region, thus validating our method.}
% \label{fig:visscore}
% \end{figure}

% M3DRef-CLIP on Imputed ScanRefer
% \begin{center}
% \begin{tabular}{ c | c  c  c }
% &Overall  & Unique & Multiple \\
%  \hline
%  50\% IOU & cell5 & cell6 \\  
%  25\% IOU & cell8 & cell9    
% \end{tabular}
% \end{center}

% M3DRef-CLIP+ on Imputed ScanRefer (All Modules Except Matching Module Frozen)
% \begin{center}
% \begin{tabular}{ c | c  c  c }
% &Overall  & Unique & Multiple \\
%  \hline
%  50\% IOU & cell5 & cell6 \\  
%  25\% IOU & cell8 & cell9    
% \end{tabular}
% \end{center}

% M3DRef-CLIP+ on Imputed ScanRefer (All Modules Except Matching Module Frozen)
% \begin{center}
% \begin{tabular}{ c | c  c  c }
% &Overall  & Unique & Multiple \\
%  \hline
%  50\% IOU & cell5 & cell6 \\  
%  25\% IOU & cell8 & cell9    
% \end{tabular}
% \end{center}

==> sec/Discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\noindent\textbf{Optimizing gesture-enhanced 3D grounding for reducing processing latency and energy overheads: } Our proposed \namess approach facilitates accurate 3D grounding even in the presence of human pointing gestures. However, Weerakoon et al. have demonstrated that the presence of pointing gestures in 2D visual grounding can reduce latency and energy overheads~\cite{COSM2IC}. 
Their key principle involves assessing task complexity through inexpensive computations, such as determining if a scene is cluttered with objects (indicating higher task complexity), and subsequently employing an appropriate execution pipeline tailored to comprehend the instruction efficiently. 
We believe that this principle of reducing computational latency and energy consumption by strategically augmenting the execution pipeline is particularly well-suited for 3DREC, especially within large point clouds. 
As the complexity of 3DREC may escalate with the volume of points in the scene, it becomes feasible to narrow down the search space for REC by identifying the pointing direction. 
This allows us to limit resource-intensive operations to a specific area of interest within the pointing direction. 
By adopting this approach, we can substantially mitigate latency while maintaining comparable accuracy, particularly in expansive 3D environments.
% \noindent\textbf{Enabling more diverse and natural pointing gestures: } While the proposed \dataset dataset,  
